Anti-efficient encoding in emergent communication

Despite renewed interest in emergent language simulations with neural networks, little is known about the basic properties of the induced code, and how they compare to human language. One fundamental characteristic of the latter, known as Zipf's Law of Abbreviation (ZLA), is that more frequent words are efficiently associated to shorter strings. We study whether the same pattern emerges when two neural networks, a "speaker" and a "listener", are trained to play a signaling game. Surprisingly, we find that networks develop an \emph{anti-efficient} encoding scheme, in which the most frequent inputs are associated to the longest messages, and messages in general are skewed towards the maximum length threshold. This anti-efficient code appears easier to discriminate for the listener, and, unlike in human communication, the speaker does not impose a contrasting least-effort pressure towards brevity. Indeed, when the cost function includes a penalty for longer messages, the resulting message distribution starts respecting ZLA. Our analysis stresses the importance of studying the basic features of emergent communication in a highly controlled setup, to ensure the latter will not strand too far from human language. Moreover, we present a concrete illustration of how different functional pressures can lead to successful communication codes that lack basic properties of human language, thus highlighting the role such pressures play in the latter.

==> intermittentsilence.tex <==
\subsection{Intermittent silence baseline} 
We want to compare the emergent language with a monkey typing baseline that would map each of the inputs to a single message. Imagine that a monkey hits the keys of a typewriter of $V$ keys at random, subject to these constraints:
\begin{enumerate}
\item the monkey hits any key with a uniform probability of $p=\frac{1}{V}$.
\item the message stops when the space key; -$\texttt{eos}$,  is hit.
\item a message cannot be longer to a specific length $\texttt{max_len}$.
\item a message should be mapped to a unique input. If the monkey constructs a message that has already been assigned to another input, he repeats the process.
\end{enumerate}

This baseline is similar to the intermittent silence baseline introduced by \cite{miller} with the extra constraints of the $\texttt{max_len}$ and the uniform probability over the keys. Intuitively, we think that without any prior, this baseline should be the one developed by the agent sender. Interestingly, this baseline is know to follow the `Zipf's Law' without any deliberate effort to do so \cite[]{miller}. In other words, we can predict that, without any specific biases, the sender-receiver system would come up with a language following the Zipfian distribution.

In the monkey's output we will find messages of $l$ symbols, where $l = 1, 2, \ldots, \texttt{max_len}$. We will expect to find runs of length $l$ with a probability

$$P_l=p \times (1- p)^{l-1}, \mbox{if } l<\texttt{max_len} \mbox{ and } P_{\texttt{max_len}}=(1- p)^{\texttt{max_len}-1} $$

Hence, to construct this baselines, we first sample, for a given input, a length according to the defined length distribution and then sample uniformally from $V \setminus \{ eos \}$. We repeat this process until having a unique message for each input.

==> relatedworks.tex <==
\section{Related work} 

\paragraph{Word length distributions in natural language} In his
pioneering studies of lexical statistics (see in particular
\cite{Zipf:1949}), George Kingsley Zipf noticed a robust trend in
human language that came to be known as Zipf's Law of Abbreviation
(ZLA): More frequent words always tend to be shorter, with a roughly
log-linear inverse correlation between frequency and length
\citep{Strauss:etal:2007}. \textbf{Once we have the human-data plots,
  we could actually refer to them here.} Assuming that shorter words
are easier to produce, this is an efficient encoding strategy,
particularly effective given Zipf's other important discovery that
word distributions are highly skewed, such that a few frequent words
account for a large portion of running text and speech. Indeed, in
this way language approaches an optimal code in information-theoretic
terms \citep{Cover:Thomas:2006}. Zipf, and many after him, have thus
used ZLA as evidence that language is shaped by functional pressures
toward effort minimization
\citep[e.g.,][]{Mahowald:etal:2018,Gibson:etal:2019}. However, others
\citep[e.g.,][]{miller,ferrer2011,moscoso2013} have emphasized how
some random-typing distributions also lead to ZLA. This casts doubts
on functional explanations of the observed pattern. Our study
illustrates the emergence of a successful communication system that
does \emph{not} exhibit ZLA, suggesting that its universal presence in
human language is more interesting than what argued by the latter
studies. In particular, the lack of a speaker preference for brevity
(for a recurrent network, it is not more effortful to generate 10
characters than it is to generate one) leads to \emph{maximize} string
length, especially for the most frequent words. This might be the
result of an unconstrained discriminability pressure from the
listener. Interestingly, \cite{kanwal2017}, who ran human miniature
language experiments, found that, in conditions in which speakers can
pick longer strings at no extra cost, they will do so, in order to
ease listener accuracy.


\paragraph{Analysis of emergent communication in neural networks}
Together with a revival of language emergence simulations, there has
recently been widespread interest in studying the properties of the
emergent language
\citep[e.g.,][]{Kottur:etal:2017,Lazaridou:etal:2017,
    Bouchacourt:Baroni:2018,Evtimova:etal:2018,Lazaridou:etal:2018,Graesser:etal:2019}. With
  respect to this related literature, we focus on a narrower, more
  controlled setup, to explore the relation between input frequency
  and message length. Note that, despite the fact that extremely
  skewed concept frequency distributions are a universal property of
  language \citep{Zipf:1949,Baayen:2001}, previous work has focused on
  environments where agents need to refer to concepts with
  approximately uniform probability. The power-law input distribution
  we use makes signaling games considerably harder, as agents must be
  able to refer to concepts they encounter very rarely.


  
